Class Diagram Restructuring with GROOVE

This paper describes the GROOVE solution to the "Class Diagram Restructuring" case study of the Tool Transformation Contest 2013. We show that the visual rule formalism enables the required restructuring to be formulated in a very concise manner. Moreover, the GROOVE functionality for state space exploration allows checking confluence. Performance-wise, however, the solution does not scale well.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.10}{10.4204/EPTCS.135.10}}
\pdfoutput=1

